The SeaLion has Landed: An IDE for Answer-Set Programming---Preliminary Report

We report about the current state and designated features of the tool SeaLion, aimed to serve as an integrated development environment (IDE) for answer-set programming (ASP). A main goal of SeaLion is to provide a user-friendly environment for supporting a developer to write, evaluate, debug, and test answer-set programs. To this end, new support techniques have to be developed that suit the requirements of the answer-set semantics and meet the constraints of practical applicability. In this respect, SeaLion benefits from the research results of a project on methods and methodologies for answer-set program development in whose context SeaLion is realised. Currently, the tool provides source-code editors for the languages of Gringo and DLV that offer syntax highlighting, syntax checking, and a visual program outline. Further implemented features are support for external solvers and visualisation as well as visual editing of answer sets. SeaLion comes as a plugin of the popular Eclipse platform and provides itself interfaces for future extensions of the IDE.

==> command.tex <==
% !TEX root =  paper.tex
\newcommand{\ruleimp}{\mathtt{{:-}}}
\renewcommand{\ruleimp}{:\!- \ }
\newcommand{\grd}{\mathit{ground}}

\newcommand{\naf}{\ensuremath{\mathrm{not}}\xspace}
\newcommand{\sneg}[1]{\ensuremath{\neg#1}\xspace}
\newcommand{\compl}[1]{\ensuremath{\bar{#1}}}

\newcommand{\atomp}[1]{\ensuremath{\mathit{#1}\xspace}}
\newcommand{\atom}[2]{\ensuremath{\mathit{#1}(\mathit{#2})\xspace}}

\newcommand{\OntoStudio}{\texttt{OntoStudio}\xspace} 
\newcommand{\OntoDLV}{\texttt{OntoDLV}\xspace}
\newcommand{\smodels}{\texttt{Smodels}\xspace}
\newcommand{\gringo}{\texttt{Gringo}\xspace}
\newcommand{\aspide}{\texttt{ASPIDE}\xspace}
\newcommand{\lparse}{\texttt{Lparse}\xspace}
\newcommand{\aspviz}{\texttt{ASPVIZ}\xspace}
\newcommand{\idpdraw}{\texttt{IDPDraw}\xspace}
\newcommand{\igrom}{\texttt{iGROM}\xspace}
\newcommand{\ape}{\texttt{APE}\xspace}
\newcommand{\clasp}{\texttt{Clasp}\xspace}
\newcommand{\dlv}{\texttt{DLV}\xspace}
\newcommand{\nomore}{\texttt{noMoRe}\xspace}
\newcommand{\sealion}{\texttt{SeaLion}\xspace}
\newcommand{\kara}{\texttt{Kara}\xspace}
\newcommand{\inter}{\ensuremath{I}\xspace}
\newcommand{\ninter}{\ensuremath{N}\xspace}
\newcommand{\deltaR}{\ensuremath{{\mathit{R}_\Delta}}\xspace}
\newcommand{\deltaI}{\ensuremath{{\mathit{I}_\Delta}}\xspace}
\newcommand{\loopS}{\ensuremath{\Gamma}\xspace}
\newcommand{\opsym}[1]{\ensuremath{\Upsilon_{#1}}\xspace}
\newcommand{\op}[2]{\ensuremath{\opsym{#1}({#2})}\xspace}
%\newcommand{\statei}[1]{\ensuremath{\mathit{I}_{#1}}\xspace}
\newcommand{\statei}[1]{\ensuremath{\mathit{I}({#1})}\xspace}
\renewcommand{\statei}[1]{\ensuremath{\mathit{Int}[{#1}]}\xspace}
\newcommand{\stater}[1]{\ensuremath{\mathit{R}_{#1}}\xspace}
\newcommand{\abdtrans}[2]{\ensuremath{\lambda({#1},{#2})}\xspace}
\newcommand{\cset}{\ensuremath{C}\xspace}
\newcommand{\state}{\ensuremath{S}\xspace}
\newcommand{\facts}{\ensuremath{F}\xspace}
\newcommand{\computation}{\ensuremath{\mathrm{C}}\xspace}
\newcommand{\blockedLiterals}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\applrules}{\ensuremath{R}\xspace}
\newcommand{\activatedRules}[2]{\ensuremath{\mathit{AR}_{#2}(#1)}\xspace}

\newcommand{\intconstraints}[1]{\ensuremath{\mathit{Con}_{#1}}\xspace}

\newcommand{\activerules}[2]{\ensuremath{\mathit{Act}^{#1}({#2})}\xspace}

\newcommand{\forbidden}{\ensuremath{\mathit{forbidden}}\xspace}
\newcommand{\currentSupport}[1]{\ensuremath{\mathit{Sup}[{#1}]}\xspace}
\newcommand{\pool}{\ensuremath{\mathit{pool}}\xspace}
\newcommand{\hcpool}{\ensuremath{\mathit{pool^{HC}}}\xspace}
\newcommand{\constraintset}{\ensuremath{\mathit{Con}}\xspace}
\newcommand{\hclits}{\ensuremath{\mathbb{L}}\xspace}
\newcommand{\Pol}{{\rm P}\xspace}
\newcommand{\PNP}{\Pol^{\rm NP}\xspace}
\newcommand{\NP}{\mbox{\rm NP}\xspace}
\newcommand{\NPNP}{\NP^{\rm NP}\xspace}
\newcommand{\CONP}{\mbox{\rm coNP}\xspace}
\newcommand{\coNP}{\mbox{\rm coNP}\xspace}
\newcommand{\SigmaP}[1]{\ensuremath{{\Sigma}_{#1}^{P}}\xspace}
\newcommand{\PiP}[1]{\ensuremath{{\Pi}_{#1}^{P}}\xspace}
\newcommand{\DeltaP}[1]{\ensuremath{{\Delta}_{#1}^{P}}\xspace}

\newcommand{\lang}{\ensuremath{\mathcal{L}}\xspace}

\newcommand{\la}{\ensuremath{\leftarrow}\xspace}
\newcommand{\ra}{\ensuremath{\rightarrow}\xspace}
\newcommand{\at}[1]{\ensuremath{\mathit{At}(#1)}\xspace}

\newcommand{\subst}{\ensuremath{\vartheta}\xspace}

\newcommand{\succeeds}[1]{\ensuremath{\succ_{#1}}\xspace}
\renewcommand{\succeeds}[1]{\ensuremath{\prec_{#1}}\xspace}
\newcommand{\result}[1]{\ensuremath{\mathit{res}({#1})}\xspace}

\newcommand{\be}{\begin{compactenum}}
\newcommand{\ee}{\end{compactenum}}
\newcommand{\bi}{\begin{compactitem}}
\newcommand{\ei}{\end{compactitem}}

\newcommand{\AS}[1]{\ensuremath{\mathit{AS}(#1)}\xspace}
\newcommand{\SM}[1]{\AS{#1}}

\newcommand{\naturals}[0]{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\vhack}{\vspace{-8pt}}
\newcommand{\vhackafter}{\vspace{-5.5pt}}
\renewcommand{\vhack}{}
\renewcommand{\vhackafter}{}
\newcommand{\lit}[1]{\ensuremath{\mathit{L}(#1)}\xspace}


\newcommand{\hcfuncsym}[2]{\ensuremath{f_{#1,#2}}\xspace}
\newcommand{\hcfunc}[3]{\ensuremath{\hcfuncsym{#1}{#2}({#3})}\xspace}

\newcommand{\viz}[0]{viz.\xspace}
\newcommand{\wrt}[0]{with respect to\xspace}
%\newcommand{\wrt}[0]{w.r.t.\xspace}
\newcommand{\iec}[0]{i.e.,\xspace}
\newcommand{\Iec}[0]{I.e.,\xspace}
\newcommand{\egc}[0]{e.g.,\xspace}
\newcommand{\eg}[0]{e.g.\xspace}
\newcommand{\resp}[0]{resp.,\xspace}
\newcommand{\nop}[1]{}
\newcommand{\body}[1]{\ensuremath{\mathrm{B(}{#1}\mathrm{)}}\xspace}
\newcommand{\head}[1]{\ensuremath{\mathrm{H(}{#1}\mathrm{)}}\xspace}
\newcommand{\pbody}[1]{\ensuremath{\mathrm{{B^+}(}{#1}\mathrm{)}}\xspace}
\newcommand{\nbody}[1]{\ensuremath{\mathrm{{B^-}(}{#1}\mathrm{)}}\xspace}
\newcommand{\gr}[1]{\ensuremath{\mathit{gr(}{#1}\mathit{)}}\xspace}
\newcommand{\tupel}[1]{\ensuremath{\langle {#1} \rangle}\xspace}
\newcommand{\set}[1]{\ensuremath{\{{#1}\}}\xspace}
\newcommand{\abs}[1]{\ensuremath{|{#1}|}\xspace}
\newcommand{\selfsupp}[0]{self-supporting\xspace}
\newcommand{\stable}[0]{stable\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

